Camels in a Changing Climate: Enhancing LM Adaptation with Tulu 2

Since the release of T\"ULU [Wang et al., 2023b], open resources for instruction tuning have developed quickly, from better base models to new finetuning techniques. We test and incorporate a number of these advances into T\"ULU, resulting in T\"ULU 2, a suite of improved T\"ULU models for advancing the understanding and best practices of adapting pretrained language models to downstream tasks and user preferences. Concretely, we release: (1) T\"ULU-V2-mix, an improved collection of high-quality instruction datasets; (2) T\"ULU 2, LLAMA-2 models finetuned on the V2 mixture; (3) T\"ULU 2+DPO, T\"ULU 2 models trained with direct preference optimization (DPO), including the largest DPO-trained model to date (T\"ULU 2+DPO 70B); (4) CODE T\"ULU 2, CODE LLAMA models finetuned on our V2 mix that outperform CODE LLAMA and its instruction-tuned variant, CODE LLAMA-Instruct. Our evaluation from multiple perspectives shows that the T\"ULU 2 suite achieves state-of-the-art performance among open models and matches or exceeds the performance of GPT-3.5-turbo-0301 on several benchmarks. We release all the checkpoints, data, training and evaluation code to facilitate future open efforts on adapting large language models.

==> tables/main_table.tex <==
% rows of table:
% tulu2, codetulu2, base llama2, llama2-chat, Code-LLaMa2-Instruct
% good to test: zephyr, xwin, any others?
\begin{table}[htbp]
\centering
\caption{
The evaluation metrics of our core \modelname{}-V2 suite and its peers.
Most of the models included use \llama~2 or \codellama~base models, except Zephyr-$\beta$ that uses \mistral-7B. 
For all evaluations except ToxiGen, higher scores are better.
\textcolor{red}{todo: remove truthfulqa? grey it out? remove it from avg?}
}
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccc}
\toprule
{} & MMLU  & GSM8k & BBH  & TydiQA GP & CodexEval & AlpacaEval & ToxiGen & TruthfulQA & Average \\
{} & 0-shot, EM & CoT, 8-shot, EM & CoT, 3-shot, EM & 1-shot, F1 & P@10 & \% Win & \% Toxic & \%Info+\%True & - \\
\midrule
\multicolumn{9}{c}{Proprietary models ↓} \\ \midrule
GPT-4-0314  & 82.4 & 92.5 & 88.0 &  70.8 & 94.1 & 93.5 &  10.6 & 82.3 & 86.6 \\
ChatGPT-turbo-0301 & 67.9 & 76.0 & 66.1 &  51.9 & 88.4 &  83.6 &  27.7 & 75.2 & 72.7 \\
\midrule
\multicolumn{9}{c}{\llama 7B finetuning experiments ↓} \\ \midrule
\llama 7B vanilla & 41.8 & 12.0 & 39.3 & 51.2 & 26.8 && 77.3 & 26.7 & - \\
\modelname~V1 & 49.2 & 37.0 & 44.2 & 52.9 & 33.9 & 57.3 & 39.9 & 40.8 & 46.9 \\
\llama-Chat & 46.8 & 12.0 & 25.6 & 22.7 & 24.0 & 79.4 & 0.0 & 22.6 & 41.6 \\
\modelname~V2 UltraFDPO & 50.7 & 34.5 & 45.5 & 44.5 & 40.0 & 76.7 & 0.5 & 67.4 & 57.3 \\
Zephyr-Beta 7B* \\
ShareGPT &&&& && 66.1 && \\
ShareGPT+UltraPref &&&& && 75.8 && \\
\modelname~V2 (QLoRA) & 48.8 & 20.5 & 45.7 & 49.2 & 31.7 & 51.7 & 14.7 & 44.6 & 47.2 \\
\modelname~V2 & 50.4 & 34.0 & 48.5 & 46.4 & 36.9 & 67.3 & 7.0 & 50.2 
 & 53.3 \\\midrule
\multicolumn{9}{c}{\llama 13B finetuning experiments ↓} \\\midrule
\llama 13B vanilla & 52.0 & 25.0 & 48.9 & 56.5 & 32.5 && 85.7 & 31.1 & - \\
\modelname~V1 & 52.3 & 53.0 & 50.6 & 58.8 & 38.9 & 64.0 & 18.7 & 45.3 & 55.5 \\
\llama-Chat & 53.2 & 9.0 & 40.3 & 32.1 & 33.1 & 86.8 & 0.0 & 44.7 \\
\modelname~v2 UltraFDPO & 55.3 & 49.5 & 49.4 & 39.7 & 48.9 & 82.9 & 1.1 & 70.0 & 61.8 \\
\modelname~V2 (QLoRA) & 54.6 & 36.0 & 52.5 & 54.6 & 39.1 & 59.8 & 0.0 & 55.2 & 56.5 \\
\modelname~V2 & 55.4 & 46.0 & 49.5 & 53.2 & 49.0 & 73.9 & 1.7 & 55.8 & 60.1 \\\midrule
\multicolumn{9}{c}{\llama 70B finetuning experiments ↓} \\\midrule
\llama 70B vanilla & 64.5 & 55.5 & 66.0 & 62.6 & 60.1 && 84.2 & 38.2 & - \\
\modelname~V1 & 67.3 & 74.5 & 66.0 & 62.6 & 65.4 & 80.2 & 0.0 & 38.2 & 69.3 \\
\llama-Chat & 60.9 & 59.0 & 49.0 & 44.4 & 52.1 & 89.3 & 0.0 & 59.6 & 64.3 \\
Xwin-LM v0.2 70B \\
\modelname~V2 UltraFDPO   &&&&  && 91.9 &    &    \\
\modelname~V2 (QLoRA) & 67.4 & 64.5 & 71.6 & 60.9 & 66.9 & 76.6 & 0.5 & 58.4 & 70.7 \\
\modelname~V2 & 67.3 & 73.0 & 68.4 & 53.6 & 68.5 & 84.3 & 0.5 & 62.2 & 72.1 \\\midrule
\multicolumn{9}{c}{\codellama 7B finetuning experiments ↓} \\\midrule
\codellama 7B vanilla & 33.8 & 12.0 & 43.4 & 47.6 & 58.7 && 81.5 & 26.1 & 34.3 \\
\codemodelname~V2 & 43.7 & 33.0 & 49.1 & 52.6 & 68.9 & 54.0 & 5.0 & 33.0 & 53.7 \\
\codellama-Instruct & 41.5 & 17.0 & 38.4 & 41.6 & 64.1 & 61.7 & 1.0 & 15.2 & 47.3 \\\midrule
\multicolumn{9}{c}{\codellama 13B finetuning experiments ↓} \\\midrule
\codellama 13B vanilla & 37.5 & 22.0 & 49.5 & 52.1 & 69.8 && 77.9 & 26.9 & 40.0 \\
\codemodelname~V2 & 45.9 & 41.0 & 52.8 & 55.7 & 76.2 & 58.4 & 0.0 & 36.7 & 58.3 \\
\codellama-Instruct & 43.3 & 23.0 & 48.0 & 37.8 & 69.2 & 64.5 & 0.0 & 38.1 & 53.0 \\\midrule
\multicolumn{9}{c}{\codellama 34B finetuning experiments ↓} \\\midrule
\codellama 34B vanilla & 47.4 & 35.0 & 57.0 & 57.1 & 77.6 && 88.3 & 24.4 & 44.3 \\
\codemodelname~V2 & 53.6 & 54.0 & 64.3 & 60.6 & 82.5 & 72.0 & 0.0 & 42.0 & 66.1 \\
\codellama-Instruct & 50.9 & 38.0 & 59.2 & 55.1 & 76.5 & 78.1 & 0.0 & 51.2 & 63.6 \\

\bottomrule
\end{tabular}

}
\end{table}
